DANCE: Detect and Classify Events in EEG

Event identification in continuous neural recordings is a critical task in neuroscience. Decoding in EEG is dominated by classifying windows aligned to known event onsets. However, while available in controlled experiments, such onsets are absent in continuous real-world monitoring. Here, we introduce DANCE, a deep learning pipeline that frames neural decoding as a set-prediction problem and jointly detects and classifies events directly from raw, unaligned signals. Evaluated separately on ten datasets curated from the literature with a wide variety of event types (ranging from milliseconds to minutes in duration), our model outperforms existing methods on a broad range of cognitive, clinical and BCI tasks. This single architecture establishes a new state of the art in the competitive task of seizure monitoring and matches the accuracy of onset-informed models for BCI tasks. Overall, our method marks a step towards end-to-end asynchronous neural decoding models

==> Makefile <==
MAIN ?= dance_meta.tex
BASE := $(basename $(MAIN))

# Default: build the PDF using the checked-in dance_meta.bbl (no bibtex run).
all: $(BASE).pdf

$(BASE).pdf: $(MAIN) dance_meta.bbl
	BSTINPUTS=.:./assets: latexmk --shell-escape --pdf -interaction=nonstopmode -file-line-error $(MAIN)

# Alternate entrypoint to build the legacy NeurIPS template version.
neurips:
	$(MAKE) MAIN=dance_neurips.tex

# Refresh dance_meta.bbl from dance_neurips.bib by temporarily reactivating
# the \bibliography{}/\bibliographystyle{} pair, running bibtex, then
# restoring the \input{dance_meta.bbl} form. Use this after editing the .bib.
refresh-bbl:
	@echo ">> Refreshing dance_meta.bbl from dance_neurips.bib..."
	@cp dance_meta.tex .dance_meta.tex.bibtex-bak
	@/usr/bin/python3 -c "p='dance_meta.tex'; s=open(p).read(); s=s.replace('\\\\input{dance_meta.bbl}', '\\\\bibliographystyle{plainnat}\\n\\\\bibliography{dance_neurips}'); open(p,'w').write(s)"
	@BSTINPUTS=.:./assets: latexmk --shell-escape --pdf -bibtex -interaction=nonstopmode -file-line-error dance_meta.tex || true
	@mv .dance_meta.tex.bibtex-bak dance_meta.tex
	@latexmk -C dance_meta.tex >/dev/null 2>&1 || true
	@echo ">> dance_meta.bbl refreshed."

# Clean intermediates (keeps dance_meta.bbl, which is treated as a source).
clean:
	rm -f *.aux *.log *.snm *.nav *.fls *.blg *.fdb_latexmk *.out *.toc *.brf *.bcf *.run.xml *.idx *.ilg *.ind *.synctex.gz

distclean: clean
	rm -f dance_meta.pdf dance_neurips.pdf

.PHONY: all neurips refresh-bbl clean distclean

